KS-Lottery: Finding Certified Lottery Tickets for Multilingual Language Models

The lottery ticket hypothesis posits the existence of ``winning tickets'' within a randomly initialized neural network. Do winning tickets exist for LLMs in fine-tuning scenarios? How can we find such winning tickets? In this paper, we propose KS-Lottery, a method to identify a small subset of LLM parameters highly effective in multilingual fine-tuning. Our key idea is to use Kolmogorov-Smirnov Test to analyze the distribution shift of parameters before and after fine-tuning. We further theoretically prove that KS-Lottery can find the certified winning tickets in the embedding layer, fine-tuning on the found parameters is guaranteed to perform as well as full fine-tuning. Comparing KS-Lottery with other parameter-efficient tuning algorithms on translation tasks, the experimental results show that KS-Lottery finds a much smaller set of parameters for fine-tuning while achieving the comparable performance as full fine-tuning LLM. Surprisingly, we find that fine-tuning 18 tokens' embedding of LLaMA suffices to reach the fine-tuning translation performance~\footnote{https://github.com/CONE-MT/KS-Lottery.}.

==> NIPS-2024/sections/3.algorithm_backup.tex <==
\section{Certified Winning Tickets via \name}

In this section, we begin by exploring the existence of key parameters for multilingual transfer,
focusing especially on token embeddings, employing heuristic methods~(\S~\ref{sec: find winning}). Then we introduce a Kolmogorov-Smirnov Test~(KS-Test;~\citealp{ks-test}) in \S~\ref{sec: ks-test} to identify winning tickets within the model and use theoretical results~(\S~\ref{section: theory}) as well as experiments~(\S~\ref{section: exp main}) to validate the effectiveness of \name. Figure~\ref{fig:introduction_overview} shows the overview of \name.


% Comparison of parameter change before and after finetuning on Alpaca-en. 在每一层独立训练，然后每一层用我们的方法观察重点变化的参数有哪些。在横线上的点代表出现显著变化。it is observable that the significant changes体现在0-th layer(embedding layer) 以及LayerNorm layers

% 要体现的：重点变化在不同层是有差异的，其他的变化全部集中在embedding. It is observable that 在layer内的变化都集中在LayerNorm layers，while其他变化基本都集中在0-th layer(embedding layer)

\subsection{Finding Winning Tickets: a Heuristic Approach\label{sec: find winning}}
% \citet{frankle2018lottery} hypothesized that the structure and location of ``winning tickets"—subnetworks identified during the iterative pruning process—encode an inductive bias that is uniquely tailored to the learning task at hand. In a similar vein, \citet{zheng-etal-2022-robust} discovered that these winning tickets tend to be more sparsely distributed in the later layers of the BERT model when applied to GLUE tasks. Although much of this research has centered around the concept of model pruning, there has been parallel work in the domain of parameter-efficient tuning. For instance,~\citep{he2021towards} demonstrated that the performance of fine-tuned parameters at various locations within a network can reflect both the inductive biases of the tasks and the inherent structure of the model.

\noindent\textbf{Setting} Guided by the hypothesis that parameters undergoing substantial changes during fine-tuning are crucial for making predictions~\citep{levin2022models}, 
we exam the distribution $p_i$ of each parameter $\boldsymbol{\theta}_i$ (with the parameter $\theta_{ij}$ of token $j$ drawn from $p_i$) before and after the fine-tuning. 
To assess whether there has been a significant shift in the parameter distribution, we utilize the KS-Test. A lower significance level $\alpha$ indicates a significant alteration of the parameters during fine-tuning. 

\begin{table}[!hb]
    \vspace{-0.25cm}
    \centering
    \small
    \caption{The LLaMA-7B model, which consists of 32 layers excluding the embedding layer, is fine-tuned on a single layer to evaluate its average translation performance on the Flores-101 devtest. The layers are numbered based on their distance to the embedding layer, starting with Layer 0 as the closest and Layer 31 as the furthest. The term ``Layer $i$ Tunning'' indicates that only the $i$ th layer is fine-tuned, with the other parts of parameters fixed.}
    \label{tab:tuning-method}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lc|lc|lc|lc}
        \toprule
        \textbf{Setting} & \textbf{spBLEU} & \textbf{Setting} & \textbf{spBLEU} & \textbf{Setting} & \textbf{spBLEU} & \textbf{Setting} & \textbf{spBLEU} \\ 
        \midrule
        Full Tuning  & \cellcolor{mycolor!28.2} 28.2    & Layer 6 Tuning & \cellcolor{mycolor!29.3} 29.3 & Layer 15 Tuning & \cellcolor{mycolor!19.6} 19.6 & Layer 24 Tuning & \cellcolor{mycolor!3.5} 3.5 \\ 
        LoRA & \cellcolor{mycolor!29.1} 29.1            & Layer 7 Tuning & \cellcolor{mycolor!29.1} 29.1 & Layer 16 Tuning & \cellcolor{mycolor!17.2} 17.2 & Layer 25 Tuning & \cellcolor{mycolor!3.8} 3.8 \\ 
        Embed Tuning & \cellcolor{mycolor!29.2} 29.2    & Layer 8 Tuning & \cellcolor{mycolor!29.1} 29.1 & Layer 17 Tuning & \cellcolor{mycolor!18.1} 18.1 & Layer 26 Tuning & \cellcolor{mycolor!3.7} 3.7 \\ 
        Layer 0 Tuning & \cellcolor{mycolor!29.7} 29.7  & Layer 9 Tuning & \cellcolor{mycolor!28.9} 28.9 & Layer 18 Tuning & \cellcolor{mycolor!6.8} 6.8 & Layer 27 Tuning & \cellcolor{mycolor!4.0} 4.0 \\ 
        Layer 1 Tuning & \cellcolor{mycolor!29.2} 29.2  & Layer 10 Tuning & \cellcolor{mycolor!28.0} 28.0 & Layer 19 Tuning & \cellcolor{mycolor!4.3} 4.3 & Layer 28 Tuning & \cellcolor{mycolor!3.5} 3.5 \\ 
        Layer 2 Tuning & \cellcolor{mycolor!29.5} 29.5  & Layer 11 Tuning & \cellcolor{mycolor!28.2} 28.2 & Layer 20 Tuning & \cellcolor{mycolor!4.8} 4.8 & Layer 29 Tuning & \cellcolor{mycolor!4.6} 4.6 \\ 
        Layer 3 Tuning & \cellcolor{mycolor!29.2} 29.2  & Layer 12 Tuning & \cellcolor{mycolor!27.4} 27.4 & Layer 21 Tuning & \cellcolor{mycolor!3.9} 3.9 & Layer 30 Tuning & \cellcolor{mycolor!4.4} 4.4 \\ 
        Layer 4 Tuning & \cellcolor{mycolor!29.3} 29.3  & Layer 13 Tuning & \cellcolor{mycolor!27.4} 27.4 & Layer 22 Tuning & \cellcolor{mycolor!4.8} 4.8 & Layer 31 Tuning & \cellcolor{mycolor!4.1} 4.1 \\ 
        Layer 5 Tuning & \cellcolor{mycolor!29.6} 29.6  & Layer 14 Tuning & \cellcolor{mycolor!25.2} 25.2 & Layer 23 Tuning & \cellcolor{mycolor!2.9} 2.9 \\ 
        \bottomrule
    \end{tabular}}
    \vspace{-0.25cm}
\end{table}
\textbf{Identify the small parameter set required for effective multilingual transfer.} After training all model parameters using en$\rightarrow$ca bilingual sentence pair from Lego-MT~\citep{yuan-etal-2023-lego}, we utilize the KS-Test to identify a small parameter set for multilingual transfer by comparing the parameters before and after tuning. Interestingly, we find that no parameters exhibited significant changes before and after tuning. This outcome suggests that no parameter necessitates substantial adjustments for multilingual transfer. Concurrently, the study by~\cite{yuan2023multilingual} revealed that fine-tuning specific layers, including the embedding layer, can yield results comparable to those of full-tuning. 


\begin{figure}[!hb]
\centering
\subfloat[Parameter changes before and after fine-tuning \label{fig:full-ft-ks}]
{
	\includegraphics[width=0.47\textwidth]{NIPS-2024/image/whole_model_test.pdf}
}
\hspace{0.1in}
\subfloat[Token distribution\label{fig:distribution}]
{
	\includegraphics[width=0.47\textwidth]{NIPS-2024/image/distribution.pdf}
}
\caption{\textbf{(a)} Comparison of parameter change before and after fine-tuning on Lego-MT~\cite{yuan-etal-2023-lego} en$\rightarrow$ca 10k data. Each layer is trained in isolation and is analyzed using our method to identify the parameters with significant changes (as indicated by scatter points above the red line). We find that within each Transformer layer, changes are primarily focused on LayerNorm layers, while other notable changes mainly occur in the 0-th layer (embedding layer). \textbf{(b)} Displaying the distribution of a single token~(Token ID 376), before and after embedding tuning.}
\label{fig:eq_condition}
\end{figure}
\textbf{Most significant parameter shifts happen in embedding and LayerNorm.}  Figure \ref{fig:full-ft-ks} reveals that following fine-tuning on the Lego-MT~\cite{yuan-etal-2023-lego} en$\rightarrow$ca bilingual dataset, a subset of token embeddings exhibit significant changes in their parameters. Additionally, a small number of parameters (fewer than two for each layer with a significance level of $\alpha<0.05$) demonstrate substantial changes within LayerNorm. This finding aligns with intuition, considering that transfer learning in multilingual tasks tends to lean more heavily on acquiring the low-level vocabulary nuances while preserving the semantics across languages. However, for multilingual transfer, the impact of LayerNorm varies and is not uniform across the lower and higher layers. Therefore, we concentrate our analysis on the embedding layer.



\begin{wraptable}{R}{0.50\textwidth} 
\vspace{-0.4cm}
% \begin{table}[!t]
    \centering
    \footnotesize
    \caption{Comparative analysis of training strategies on LLaMA using Alpaca-En~\cite{alpaca} dataset. The results indicate that embedding tuning yields performance comparable to other tuning strategies for multilingual tasks.}
    \label{tab:part-ft_fl}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l|cccc|c}
        \toprule
        \textbf{Models} &  \textbf{XCOPA} & \textbf{MGSM} & \textbf{XNLI} & \textbf{Flores-101} & \textbf{Avg.} \\ 
        \midrule
        Parrot-7B~\citep{jiao2023parrot} & 54.2  & 3.7  & 39.0  & 25.2  & 30.5  \\ 
        LLaMA~\citep{yuan2023multilingual} & 53.9  & 5.8  & 37.1  & 4.4  & 25.3  \\ 
        \cdashline{1-6}[0.4pt/2pt]
        Full Tuning~\citep{yuan2023multilingual} & \textbf{54.5}  & 4.5  & \textbf{40.3}  & 28.2  & \textbf{31.9}  \\ 
        LoRA~\citep{hu2022lora} & 54.4  & 6.0  & 38.4  & 29.1  & 32.0  \\ 
        Embed Tuning & 54.0  & \textbf{6.2}  & 38.0  & \textbf{29.2}  & 31.9 \\ 
        \bottomrule
    \end{tabular}
    }
\vspace{-0.5cm}
% \end{table}
\end{wraptable}
\textbf{Tuning embedding alone achieves comparable performance\label{sec: ks-test}.} 
% Motivated by the previous results, we intend to find winning tickets heuristically by choosing the parameters with the most significant distributional changes. 
% However, merely tuning the LayerNorm parameter in one Transformer layer while freezing others in that layer leads to unstable training.
% Thus we focus on finding winning tickets within embedding parameters. 
We further conduct experiments on LLaMA with different training strategies using the Alpaca-En~\cite{alpaca} dataset and then % evaluate the resulting model on four benchmarks. 
evaluate on four benchmarks. 
XCOPA~\citep{ponti2020xcopa}, MGSM~\citep{shi2022language}, and XNLI~\citep{xnli} are understanding tasks, evaluated on all languages with accuracy; 
Flores-101~\citep{flores} is a generation task, each score in the cell represents an average spBLEU, encompassing bilingual translation performances from en$\rightarrow$\{ro, es, de, ca, pt, da, no, bs\}. As shown in Figure~\ref{fig:selection} and Table~\ref{tab:part-ft_fl}, 
the empirical results
% experimental findings 
indicate that the efficacy of embedding tuning matches that of full tuning and other parameter-efficient approaches.
Thus it is safe to assume there exists a set of winning tickets within the embedding layer. 

\begin{assumption}(Winning Tickets within Embedding Layer)
    There exists a set of winning tickets $\boldsymbol{\theta}_a^E$ within the token embeddings $\boldsymbol{\theta}^E=[\theta_0, \theta_1, \cdots, \theta_{|V|}]$, where $\boldsymbol{\theta}^E=[\boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E]$, $\widetilde{\boldsymbol{\theta}}^E=[\widetilde{\boldsymbol{\theta}}_a^E, \boldsymbol{\theta}_b^E]$ is the parameters of embedding layer before and after tuning. If tuning on parameters $\boldsymbol{\theta}_a^E$ would achieve similar performance to full tuning on $\boldsymbol{\theta}^E$ downstream tasks, then we refer to $\boldsymbol{\theta}^E$ as the winning tickets of the embedding layer. For convenience, we discuss the downstream task as a next-token prediction problem, which is central to text generation, such that for an LLM~$f(\cdot, \boldsymbol{\theta}^E)$, given input context $x$, generate the most probable token in vocabulary set $\mathcal{Y}$.
\begin{equation}
    \begin{aligned}
        &g(x, \widetilde{\boldsymbol{\theta}}_a^E, \boldsymbol{\theta}_b^E) = g(x, \widetilde{\boldsymbol{\theta}}_a^E, \widetilde{\boldsymbol{\theta}}_b^E), 
        \\&\text{where} \ g(x, \boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E) = arg\max_{c\in \mathcal{Y}}\mathbb{P}\left[f(x, \boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E) = c \right]
    \end{aligned}
    \label{problem definition}
\end{equation} 
\end{assumption}

% Generally, fine-tuning LLMs on the downstream task can equip them with specialized capabilities. This process can be represented by a transition in $M$ parameters from $\boldsymbol{\theta} = [\theta_0, \theta_1, \cdots, \theta_M]$ to $\boldsymbol{\widetilde{\theta}} = [\widetilde{\theta}_0, \widetilde{\theta}_1, \cdots,  \widetilde{\theta}_M]$, where  $\boldsymbol{\theta}$ and $\boldsymbol{\widetilde{\theta}}$ denote the sets of parameters that characterize the LLM $f(\cdot, \boldsymbol{\theta})$ before and after the fine-tuning process, respectively. Notably, previous literature in parameter-efficient tuning~\citep{houlsby2019parameter,liu2021gpt, li-liang-2021-prefix} indicated that efficient and effective fine-tuning could be achieved by only altering a small subset of the parameters~($\widetilde{\boldsymbol{\theta}}^D =  [\widetilde{\theta}_0, \widetilde{\theta}_1, \cdots, \widetilde{\theta}_D, \theta_{D+1}, \cdots, \theta_M]$), where $D\ll M$. In the context of multilingual language models~(LLMs), a significant portion of the parameters is concentrated in the embedding layer and we intend to investigate parameter-efficient tuning from an embedding layer perspective.

% Intriguingly, recent research by~\citet{yuan2023multilingual} suggests that the multilingual capabilities inherent to Indo-European languages can be activated merely by fine-tuning the embedding layer of an LLM. This marks the strong transfer potential of embedding parameters in multilingual LLMs. However, this embedding space is still quite large, with over 32k $\times$ 4096 parameters in a Llama model. Therefore, we intend to investigate the potentials of parameter-efficient finetuning through selective token embeddings by answering two questions (1) Is embedding finetuning enough for LLM to have multilingual abilities? (2) Can we select a small subset of the tokens for finetuning to reduce the computation overhead? 

% \paragraph{Embedding Tuning Achieves Comparable Performance\label{sec: ks-test}} We further conduct an experiment on Llama with different training strategies using the Alpaca-En dataset and then evaluate the resulting model on four benchmarks. XCOPA~\citep{ponti2020xcopa}, MGSM~\citep{shi2022language}, and XNLI~\citep{xnli} are understanding tasks, evaluated on all languages with accuracy metric; Flores-101~\citep{flores} is a generation task, each score in the cell represents an average spBLEU, encompassing bilingual translation performances from en$\rightarrow$\{ro, es, de, ca, pt, da, no, bs\}. As shown in Table~\ref{tab:part-ft_fl}, the experimental findings indicate that the efficacy of embedding tuning matches that of full fine-tuning and other parameter-efficient tuning.


% \begin{figure}[t!]
% 	\centering
% 		\includegraphics[width=\linewidth]{ICML-2024/image/whole_model_test.pdf}
% 		\caption{Comparison of parameter change before and after fine-tuning on Lego-MT~\cite{yuan-etal-2023-lego} en$\rightarrow$ca 10k data. 
%   Each layer is trained in isolation and is analyzed using our method to identify the parameters with significant changes (as indicated by scatter points above the red line).
%   % The scatter points above the red line indicate substantial changes.
%   % It is observable that within each Transformer layer, changes are predominantly concentrated in LayerNorm layers, while other significant changes mainly occur in the 0-th layer (embedding layer).
%   We find that within each Transformer layer, 
%   changes are primarily focused on LayerNorm layers, 
%   while other notable changes mainly occur in the 0-th layer (embedding layer).
%   }
% 	\label{fig:full-ft-ks}
% \end{figure}


% \begin{figure}[t] 
% \begin{minipage}{0.48\linewidth}
% 	\centering
% 		\includegraphics[width=\linewidth]{ICML-2024/image/whole_model_test.pdf}
% 		\caption{Comparison of parameter change before and after fine-tuning on Lego-MT~\cite{yuan-etal-2023-lego} en$\rightarrow$ca 10k data. 
%   Each layer is trained in isolation and is analyzed using our method to identify the parameters with significant changes (as indicated by scatter points above the red line).
%   % The scatter points above the red line indicate substantial changes.
%   % It is observable that within each Transformer layer, changes are predominantly concentrated in LayerNorm layers, while other significant changes mainly occur in the 0-th layer (embedding layer).
%   We find that within each Transformer layer, 
%   changes are primarily focused on LayerNorm layers, 
%   while other notable changes mainly occur in the 0-th layer (embedding layer).
%   }
% 	\label{fig:full-ft-ks}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\linewidth}
% 	\centering
% 		\includegraphics[width=0.95\linewidth]{ICML-2024/image/distribution.pdf}
% 		\caption{Displaying the distribution of a single token~(Token ID 376), before and after embedding tuning.}
% 	\label{fig:distribution}
% \end{minipage}
% \end{figure}




\paragraph{Use the Kolmogorov-Smirnov Test to uncover winning tickets in a limited embedding subset.}
In light of our previous discussion, we aim to devise a method to uncover winning tickets—the most impactful parameters—within the embedding layer of LLMs like LLaMA, which boasts a vocabulary size of approximately 32k tokens. Our objective is to determine whether an even smaller subset of these parameters can be identified as winning tickets. 

% Existing works mainly rely on score-based methods to identify notable parameter change, e.g. use Cosine Similarity to choose parameters with a large change in value, $\mathrm{cos}(\widetilde{\theta}_i^E, \theta_i^E)<\tau$, where $\tau$ is a threshold. 
% % The selection results are sensitive to threshold $\tau$ and it is difficult to determine the minimum significant token embeddings necessary for the task as it is dependent on the inherent inductive bias of tasks. To actively determine the intrinsic dimension, we propose a probing strategy that employs the Kolmogorov-Smirnov Test.  
% The outcomes are sensitive to $\tau$ and is hard to determine the minimum significant token embeddings necessary for the task as it is dependent on the tasks' inherent inductive bias. 

To actively identify, we propose a probing strategy that employs the Kolmogorov-Smirnov Test, which is a statistical method used to compare two sample distributions and determine whether they are drawn from the same underlying distribution. Specifically, we view the embedding of each LLM token $j$ as a distribution as shown in Figure \ref{fig:distribution}, i.e. $\theta_{ij}^E \sim p_i$. The cumulative distribution function~(CDF) of $\theta_i^E$ and $\widetilde{\theta}_i^E$ could be denoted by $\Phi_i(\theta)$ and $\widetilde{\Phi_i}(\theta)$. The Kolmogorov-Smirnov distance between the two CDFs is 
\begin{equation}
    D_i = \sup_{\theta}|\widetilde{\Phi_i}(\theta) - \Phi_i(\theta)|
\end{equation}

% \begin{figure}[t!]
% 	\centering
% 		\includegraphics[width=0.95\linewidth]{ICML-2024/image/distribution.pdf}
% 		\caption{Displaying the distribution of a single token~(Token ID 376), before and after embedding tuning.}
% 	\label{fig:distribution}
%  % \vspace{-0.4cm}
% \end{figure}

Now we wish to determine whether a token embedding before and after fine-tuning comes from the same distribution. 
Formally, we state Kolmogorov-Smirnov Test as:
\begin{theorem}(Kolmogorov-Smirnov Test, ~\citet{ks-test}) The test statistic for this  Kolmogorov-Smirnov Test can be defined in terms of two hypotheses:
    \\
    $H_0$: $\theta_i$ and $\widetilde{\theta_i}$ come from the same distribution.\\
    $H_1$: the two samples are not from the same distribution.

If test T: $D_i >\tau(\alpha)$ is passed, then $H_1$ holds with confidence $1-\alpha$,
where $D_i = \sup_{\theta}|\widetilde{\Phi_i}(\theta) - \Phi_i(\theta)|$, $\tau(\alpha)=c(\alpha)\sqrt{\frac{2}{d}}$, the value of $c(\alpha)$ is given in the reference table~\cite{ks_reference}, and $d$ is the parameter dimension.

\label{theorem: ks-test}

\end{theorem}

Based on the Kolmogorov-Smirnov Test, we came to propose our method, KS-Lottery.

\noindent\textbf{KS-Lottery} A token embedding is designated as a ``winning ticket" if it satisfies the condition where the null hypothesis~(that there is no difference in the distribution of the embedding before and after fine-tuning) is rejected, and the alternative hypothesis $H_1$ (indicating a significant distributional change) is accepted. Kolmogorov-Smirnov Test ensures that if the distribution of token embedding $\theta_i$ does not change after fine-tuning, then $\mathbb{P}\left[D_i>\tau(\alpha)\right]<\alpha$, ensuring the majority of crucial token embeddings would be chosen by the test. 

\begin{figure}[t!]
	\centering
		\includegraphics[width=1\linewidth]{NIPS-2024/image/certified_token_selection_one_row.pdf}
		\caption{Illustration of $f(\cdot, \boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E)$ in 2 dimensions. \textbf{Left:} The concentric circles are the density contours of embedding parameters before and after fine-tuning, and the colored landscape is the decision boundaries of $f(\cdot)$. \textbf{Right:} the distribution $\mathbb{P}\left[f(x,\theta_a^E,\widetilde{\theta_b^E})\right]$ and $\mathbb{P}\left[f(x,\widetilde{\theta_a^E},\theta_b^E)\right]$. $\underline{p_A}$ is the probability 
$\mathbb{P}\left[f(x,\widetilde{\theta}_a^E,\widetilde{\theta_b^E})\right]$ predicts $x$ to be token $c_A$~(color blue), and $\overline{p_B}$ as the probability of second most likely prediction (color red). $D_{ks}$ denotes the Kolmogrov-Smirnov distance between distributions before and after tuning.
We choose the set of token embeddings for fine-tuning as those with little distribution overlap before and after fine-tuning, which may lead to significant differences in prediction. }
	\label{fig:certification intuition}
\end{figure}


\subsection{\name Finds Certifiable Winning Tickets\label{section: theory}}

Suppose that when the LLM $f(\cdot, \boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E)$ predicts any given input $x$, the most probable token $c_A$ is returned with probability $p_A$. Following the idea in randomized smoothing~\citep{muravev2021certified, zhao2022certified} that small changes to parameters in a smooth subspace do not affect decision boundary, we could probably guarantee that training on our \name selected token embeddings could achieve the same performance as full embedding layer tuning at high confidence. The intuition of the theory is illustrated in Figure \ref{fig:certification intuition}. Our main theoretical results are as follows, the proofs can be found in Appendix~\ref{appendix:proofs}: 
\begin{theorem}(Certified Winning Tickets) Let $f(\cdot, \boldsymbol{\theta}_a, \boldsymbol{\theta}_b): \mathbb{R}^d \rightarrow \mathcal{Y}$ be any random or deterministic function, and let $g$ be defined as in Equation \ref{problem definition}. 
For any input $x$, suppose $c_A \in \mathcal{Y}$, the bounds of prediction based on random variable parameters $\widetilde{\boldsymbol{\theta}}_a$, $\widetilde{\boldsymbol{\theta}}_b$, $\underline{p_A}, \overline{p_B} \in[0,1]$ satisfies 
\begin{equation}
\footnotesize
\begin{aligned}
    \mathbb{P}\left(f(x, \widetilde{\boldsymbol{\theta}}_a, \widetilde{\boldsymbol{\theta}}_b)=c_A\right)& \geq \underline{p_A}
    \geq \overline{p_B} \geq \max _{c \neq c_A} \mathbb{P}\left(f(x, \widetilde{\boldsymbol{\theta}}_a, \widetilde{\boldsymbol{\theta}}_b=c)\right)
\end{aligned}
\end{equation}
If the set of parameters $\boldsymbol{\theta}_b$ satisfies 
\begin{equation}
    D(\widetilde{\theta}^i_b, \theta^i_b)<\tau(\alpha)<\frac{\underline{p_A}-\overline{p_B}}{2},
    \label{distance bound}
\end{equation}
for all $i\in V_b$, the generator partial-tuned on parameters $\boldsymbol{\theta}_a$ always return token $c_A$, i.e. $g(x, \widetilde{\boldsymbol{\theta}}_a^E, \boldsymbol{\theta}_b^E)=c_A$. 
\vspace{-0.5cm}
\label{certification}
\end{theorem}
\ 

\begin{remark}(About $\boldsymbol{\theta}_a$) Theorem \ref{certification} immediately holds for \emph{Partial Transfer} setting as specified in \S~\ref{sec:more_analysis}. As for \emph{Partial Tuning} setting, we need to use the hypothesis that the value of $\widetilde{\boldsymbol{\theta}}_a$ in the embedding tuning setting and partial-tuning setting are the same for Theorem \ref{certification} to hold. This is due to $\boldsymbol{\theta}_a$ taking major effect during embedding tuning despite small changes in $\boldsymbol{\theta}_b$. We also show with empirical analysis in \S~\ref{sec:more_analysis} that $\widetilde{\boldsymbol{\theta}}_a$ in two tuning settings share the same distribution.
    
\end{remark}

% \begin{remark}(Training Landscape Smoothness V.S Intrinsic Dimension) Theorem \ref{certification} indicates that dimensions of parameters where the training landscape is smooth, i.e. $D(\widetilde{\theta}_i^b, \theta_i^b)$ is small, could be frozen during fine-tuning without hurting performance. This is in line with the intrinsic dimension hypotheses that some parameters do not impact performance and the majority of the performance gains could be achieved by parameter changes in an embedding space with reduced dimensions.
    
% \end{remark}


\begin{remark}(About $\alpha$) Practically, $\tau(\alpha)$ is small. 
% \xspace $\tau(\alpha)$ is small in practice. 
In the case of fully embedding tuned LLM that has optimal performance and produces confident prediction, $1>p_A\gg p_B>0$, we can choose small $\alpha=\tau^{-1}(\frac{p_A-p_B}2)$ while maintaining performance. In this case, the Kolmogorov-Smirnov Test samples fewer token embeddings for fine-tuning. 
    
\end{remark}

\begin{remark} (About Applicability) This theorem could be used for certifying fine-tuning lottery tickets for any black-box model and input. Note that \name could be applied to the entire model, though we only perform testing on the embedding layer for convenience and training stability.
    
\end{remark}

\subsection{Empirical Verification of Winning Tickets}
\label{section: exp main}

There are two different ways to verify the effectiveness of winning tickets: Partial Tuning~(sufficient condition) and Partial Transfer~(necessary condition). \noindent\textbf{Partial Tuning.} As shown in Figure~\ref{fig:introduction_overview}, only train winning tickets, keeping the remaining parameters frozen.  \noindent\textbf{Partial Transfer.}  Given a model trained by embedding tuning, we select the winning tickets from the embedding layer and use them to replace the corresponding parameters in the original model, thus curating a new model. 


As shown in Table~\ref{tab:verification}, just tuning winning tickets can achieve results on par with embedding tuning. Meanwhile,
by only modifying the winning tickets, it manages to retain $86.9\%( 31.3 / 36.1 )$ of the performance. The experimental result demonstrates that a low-dimensional subspace exists, guided by the winning tickets, that can achieve comparable performance as optimizing all parameters in the embedding-tuned model. The result empirically verifies the effectiveness of winning tickets.


\begin{table*}[!h]
    \centering
    \footnotesize
    \caption{Empirical verification of winning tickets with \textbf{Partial Tuning} and \textbf{Partial Transfer}. ~*~denotes that the random results in the table represent the average performance with three distinct seeds.}
    \label{tab:verification}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|c|ccccc||ccccc}
        \toprule
        
         \multirow{2}{*}{\textbf{\# Token}}  &  \multirow{2}{*}{\textbf{Method}}  & \multicolumn{5}{c||}{\textbf{LLaMA-7B}} & \multicolumn{5}{c}{\textbf{Mistral-7B}} \\
        & & \textbf{en$\rightarrow$ro}  &  \textbf{en$\rightarrow$es}  &  \textbf{en$\rightarrow$de}  &  \textbf{en$\rightarrow$ca } & \textbf{Avg.}  &  \textbf{en$\rightarrow$ro}  &  \textbf{en$\rightarrow$es}  &  \textbf{en$\rightarrow$de}  &  \textbf{en$\rightarrow$ca}  & \textbf{Avg.} \\ 
                \midrule
                \multicolumn{2}{c|}{Original Model}  & 3.5 & 4.8 & 4.8 & 5.7 & 4.6 &         \\ 
                \multicolumn{2}{c|}{Full Tuning} & 28.3 & 23.5 & 22.5 & 34.9 & 27.3 &       33.4 & 25.1 &29.1 & 37.8  \\ 
                \multicolumn{2}{c|}{LoRA}  & 29.8 & 26.4 & 27.8 & 37.3 & 30.3 &              \\ 
                \multicolumn{2}{c|}{Embed Tuning} & 28.7 & 25.5 & 25.8 & 36.1 & 29.0 &      34.2 & 28.3 & 33.2 & 40.2 \\ 
                \midrule
                $<$18  &  Random Tuning*   & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 &                    \\ 
                (p-value $<$ 0.05)  & Partial Tuning   & 20.7 & 26.7 & 26.4 & 37.7 & 27.9 &  \\ 
                & Partial Transfer & 23.4 & 22.6 & 16.1 & 31.1 & 23.4 &  26.7 & 27.3 & 30.5 & 37.5 \\
                \midrule
                $<$100  &  Random Tuning*    & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 &                    \\ 
                (p-value $<$ 0.25)  &  Partial Tuning & 26.9 & 27.3 & 27.2 & 37.4 & 29.7 &       \\ 
                & Partial Transfer & 25.1 & 26.5 &30.4 & 34.4 & 29.1 & 26.7 & 27.3 & 30.5 & 37.5\\
                \midrule 
                \multirow{3}{*}{$\leq$800}  &  Random Tuning*   & 5.8 & 8.7 & 5.2 & 11.8 & 7.9 &                  \\ 
                 & Partial Tuning   & 29.4 & 27.3 & 30.1 & 37.7  & 31.1 &                        \\ 
                 & Partial Transfer & 30.2 & 26.7 & 30.4 & 37.6 & 31.2 & 33.7 & 27.9 & 32.6 & 40.3 \\
        \bottomrule
    \end{tabular}}
\end{table*}


% \paragraph{Selective Token Embedding Tuning} 
% We consider a LLM with vocab set $V$, therefore the embedding parameters $\boldsymbol{\theta}^E=[\theta_0, \theta_1, \cdots, \theta_{|V|}]$, where each token embedding $\theta_i^d$ is a d dimensional vector. We aim to find a subset of the tokens $\boldsymbol{\theta}_a^E$ such that $\boldsymbol{\theta}^E=[\boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E]$, $\widetilde{\boldsymbol{\theta}}^E=[\widetilde{\boldsymbol{\theta}}_a^E, \boldsymbol{\theta}_b^E]$, fine-tuning on parameters $\boldsymbol{\theta}_a^E$ would achieve similar performance to full fine-tuning on $\boldsymbol{\theta}^E$ downstream tasks. For convenience, we discuss the downstream task as a classification problem, which could be easily extended to text generation, such that for an LLM $f(\cdot, \boldsymbol{\theta}^E)$
% \begin{equation}
%     \begin{aligned}
%         &g(x, \widetilde{\boldsymbol{\theta}}_a^E, \boldsymbol{\theta}_b^E) = g(x, \widetilde{\boldsymbol{\theta}}_a^E, \widetilde{\boldsymbol{\theta}}_b^E), 
%         \\&\text{where} \ g(x, \boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E)\\ &= arg\max_{c\in \mathcal{Y}}\mathbb{P}\left[f(x, \boldsymbol{\theta}_a^E, \boldsymbol{\theta}_b^E) = c \right]
%     \end{aligned}
%     \label{problem definition}
% \end{equation}
 
% This indicates that $\boldsymbol{\theta}_a^E$ is a subset of token embeddings that are crucial to the downstream adaptation. We intend the set of $\boldsymbol{\theta}_a^E$ to be as small as possible so as to be parameter efficient while preserving the expressiveness in finetuning. In experiments, we found that finetuning on only 18 token embeddings would be enough for Llama to gain 87\% translation performance on en$\rightarrow$ca task.

% \begin{remark} (Existence of $\boldsymbol{\theta}_a^E$) The existence of $\boldsymbol{\theta}_a^E$ with $|V_a|$ token embeddings, $|V_a|\ll |V|$ could be explained by the intrinsic dimension of multilingual tasks, expressed by
% \begin{equation}
%     \widetilde{\boldsymbol{\theta}}^E = \boldsymbol{\theta}^E + P(\widetilde{\boldsymbol{\theta}}_a^E - \boldsymbol{\theta}_a^E)
% \end{equation}
% where $P$ is a $|V|\times |V_a|$ projection matrix. Training on $\boldsymbol{\theta}^E$ could be proximated with training on a small projected space $\boldsymbol{\theta}_a^E$. The least size of the space $|V_a|$ is dependent on the language, which has varying inherent dimensions necessary to express the semantics. Through extensive empirical study,  we found that adaptation to most languages calls for less than 100 token embeddings.

% \end{remark}

% Therefore, when optimizing an LLM the difference in empirical loss~$\mathcal{P}(\cdot, \theta)$ between full fine-tuning parameterization ($\theta^F$) and embedding fine-tuning ($\theta^E$) is denoted as $\mathcal{P}_{FE} = |\mathcal{P}(\theta^F) - \mathcal{P}(\theta^E)|$. Notably, the empirical loss gap for the multilingual capabilities intrinsic to Indo-European languages is such that $\mathcal{P}_{FE} \leq \epsilon$. Why is it sufficient to simply tune the embedding layer of an LLM?


% Delving into the embedding fine-tuning, we first present the performance guarantee for the $\mathcal{P}_{E}$. Then, recognizing the difficulty in precisely identifying the root cause, we propose identification and verification algorithms to determine the parameters that are crucial in the fine-tuning of the embedding.



% Interestingly, we observe through experiments that the variance of the embeddings remains unchanged before and after fine-tuning. \chang{ref same variance test experiment}. 


% \begin{figure}[h!]
% 	\centering
% 		\includegraphics[width=1\linewidth]{ARR-2024/image/same_variance.png}
% 		\caption{token id: 376, Todo}
% 	\label{fig:same_variance}
% \end{figure}


% \begin{lemma}(Gaussian Embedding Variance Equilibrium)
% Assume token embeddings $\theta_i^E\sim \mathcal{N}(\mu, \sigma)$. For any finetuned token embeddings $\widetilde{\theta_i^E}$, the distribution of the token embeddings satisfy $\widetilde{\theta_i^E}\sim \mathcal{N}(\widetilde{\mu}, \widetilde{\sigma})$, where $\sigma = \widetilde{\sigma}$.
% \end{lemma}

% The equilibrium of the Gaussian embedding variance is largely due to the constrained change in embeddings during the fine-tuning stage, as the adjustments are more about aligning the existing distribution to better capture the nuances of the new task rather than transforming the distribution. Consequently, the cumulative distribution function (CDF) of $\theta_i^E$ and $\widetilde{\theta}_i^E$ could be denoted by $\Phi_i(\theta)$ and $\Phi_i(\theta+\delta)$, where $\Phi_i$ denotes the CDF of Gaussian distribution of $\theta_i$ and $\widetilde{\mu}=\delta + \mu$. The Kolmogorov distance between the two CDFs is expressed as 



% \begin{figure*}[h!]
% 	\centering
% 		\includegraphics[width=0.9\textwidth]{ICML-2024/image/method_overview.png}
% 		\caption{The overview of two verification method: \textbf{Partial Tuning} and \textbf{Partial Transfer}. For a given set of selected tokens, Partial Tuning only trains these tokens, ensuring other parameters remain frozen; Partial Transfer replaces the weights of these parameters in the model with the weights after embedding tuning, ensuring other parameters remain unchanged.}
% 	\label{fig:method_overview}
% \end{figure*}


==> NIPS-2024/sections/7.checklist.tex <==
\clearpage
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our abstract and introduction clearly reflect the scope and contributions of this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations are discussed in Appendix~\ref{sec:lim}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the theorems/proofs presented in this paper are accompanied by assumptions or cited relevant supporting literature.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All details regarding our empirical results are discussed in the corresponding experimental sections.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All code and data will be made public.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All details regarding our empirical results are discussed in the corresponding experimental sections.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Under the random tuning settings, we reported the averaged results across multiple seeds. For certain settings in the experiments, such as partial transfer, the results are determined. 
    We omitted the statistical details from the table to maintain a concise presentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The details of computational resources (GPUs) are discussed in Appendix~\ref{appendix_implementation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conform to the NeurIPS Code of Ethics and preserve anonymity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The potential societal impacts are discussed in Appendix~\ref{sec:lim}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Based on existing open-source language models, the contribution of this paper focuses on neuron-symbolic approaches, and will not derive risks for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The assets we used are properly cited along with the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As the contribution of this paper lies in theoretically proving that KS-Lottery can find the certified winning tickets, we do not release any new dataset in this paper. 
    Other anonymized assets (e.g., code) will be made public.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing / research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing / research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

